Few-shot Object Detection via Feature Reweighting

Conventional training of a deep CNN based object detector demands a large number of bounding box annotations, which may be unavailable for rare categories. In this work we develop a few-shot object detector that can learn to detect novel objects from only a few annotated examples. Our proposed model leverages fully labeled base classes and quickly adapts to novel classes, using a meta feature learner and a reweighting module within a one-stage detection architecture. The feature learner extracts meta features that are generalizable to detect novel object classes, using training data from base classes with sufficient samples. The reweighting module transforms a few support examples from the novel classes to a global vector that indicates the importance or relevance of meta features for detecting the corresponding objects. These two modules, together with a detection prediction module, are trained end-to-end based on an episodic few-shot learning scheme and a carefully designed loss function. Through extensive experiments we demonstrate that our model outperforms well-established baselines by a large margin for few-shot object detection, on multiple datasets and settings. We also present analysis on various aspects of our proposed model, aiming to provide some inspiration for future few-shot detection works.

==> table2.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[!t]
% \caption{Detection performance (AP) for the base and novel categories on the PASCAL VOC dataset for the first base/novel split. We evaluate the performance for different numbers of training examples for the novel categories.}
% % \footnotesize
% \centering
% \scriptsize
% \setlength\tabcolsep{3pt}
% \begin{tabular}{ll|cccccc|cccccccccccccccc}
% \toprule
%                     &             & \multicolumn{6}{c|}{Novel}               & \multicolumn{16}{c}{Base}                                                                                              \\ \hline
%                  \# Shots     &           & bird & bus  & cow  & mbike & sofa & mean & aero & bike & boat & bottle & car  & cat  & chair & table & dog  & horse & person & plant & sheep & train & tv   & mean \\ \midrule
% \multirow{4}{*}{3}  & \bs{}       & 0    & 0    & 0    & 0     & 9.1  & 1.8  & 78.0 & 77.2 & 61.2 & 45.6   & 81.6 & 83.7 & 51.7  & 73.4  & 80.7 & 79.6  & 75.0   & 45.5  & 65.6  & 83.1  & 72.7 & 70.3 \\ 
%                     & \bbsshort{} & 10.9 & 5.5  & 15.3 & 0.2   & 0.1  & 6.4  & 76.7 & 77.0 & 60.4 & 46.9   & 78.8 & 84.9 & 51.0  & 68.3  & 79.6 & 78.7  & 73.1   & 44.5  & 67.6  & 83.6  & 72.4 & 69.6 \\ %\cline{2-24} 
%                     & \bbs{}      & 21.0 & 22.0 & 19.1 & 0.5   & 0.0  & 12.5 & 73.4 & 67.5 & 56.8 & 41.2   & 77.1 & 81.6 & 45.5  & 62.1  & 74.6 & 78.9  & 67.9   & 37.8  & 54.1  & 76.4  & 71.9 & 64.4 \\ %\cline{2-24} 
%                     & \Ours{}     & 26.1 & 19.1 & 40.7 & 20.4  & 27.1 & 26.7 & 73.6 & 73.1 & 56.7 & 41.6   & 76.1 & 78.7 & 42.6  & 66.8  & 72.0 & 77.7  & 68.5   & 42.0  & 57.1  & 74.7  & 70.7 & 64.8 \\ \midrule
% \multirow{4}{*}{10} & \bs{}       & 0.0  & 0.0  & 0.0  & 0.0   & 9.1  & 1.8  & 76.9 & 77.1 & 62.2 & 47.3   & 79.4 & 85.1 & 51.3  & 70.1  & 78.6 & 78.0  & 75.2   & 47.4  & 63.9  & 85.0  & 72.3 & 70.0 \\ %\cline{2-24} 
%                     & \bbsshort{} & 11.4 & 28.4 & 8.9  & 4.8   & 7.8  & 12.2 & 77.4 & 76.9 & 60.9 & 44.8   & 78.3 & 83.2 & 48.5  & 68.9  & 78.5 & 78.9  & 72.6   & 44.8  & 67.3  & 82.7  & 69.3 & 68.9 \\ %\cline{2-24} 
%                     & \bbs{}      & 22.3 & 53.9 & 32.9 & 40.8  & 43.2 & 38.6 & 71.9 & 69.8 & 57.1 & 41.0   & 76.9 & 81.7 & 43.6  & 65.3  & 77.3 & 79.2  & 70.1   & 41.5  & 63.7  & 76.9  & 69.1 & 65.7 \\ %\cline{2-24} 
%                     & \Ours       & 30.0 & 62.7 & 43.2 & 60.6  & 39.6 & 47.2 & 65.3 & 73.5 & 54.7 & 39.5   & 75.7 & 81.1 & 35.3  & 62.5  & 72.8 & 78.8  & 68.6   & 41.5  & 59.2  & 76.2  & 69.2 & 63.6 \\ \midrule
% Full                &             & 73.4 & 78.6 & 77.6 & 78.8  & 70.7 & 75.9 & 77.9 & 78.3 & 64.4 & 45.6   & 81.8 & 87.4 & 54.0  & 71.6  & 82.0 & 80.2  & 74.6   & 47.6  & 73.8  & 83.6  & 73.1 & 71.8 \\
% \bottomrule
% \end{tabular}
% \label{tab:detail}
% \end{table*}

% \caption{The detailed results on PASCAL VOC novel split 1, with 3 and 10 shot.}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]

% \footnotesize
\centering
\scriptsize
\setlength\tabcolsep{3pt}
\begin{tabular}{ll|cccccc|cccccccccccccccc}
\toprule
                    &             & \multicolumn{6}{c|}{Novel}               & \multicolumn{16}{c}{Base}                                                                                              \\ \hline
                 \# Shots     &           & bird & bus  & cow  & mbike & sofa & mean & aero & bike & boat & bottle & car  & cat  & chair & table & dog  & horse & person & plant & sheep & train & tv   & mean \\ \midrule
\multirow{4}{*}{3}  & \bs{}       & 0    & 0    & 0    & 0     & 9.1  & 1.8  & \textbf{78.0} & \textbf{77.2} & \textbf{61.2} & 45.6   & \textbf{81.6} & 83.7 & \textbf{51.7}  & \textbf{73.4}  & \textbf{80.7} & \textbf{79.6}  & \textbf{75.0}   & \textbf{45.5}  & 65.6  & 83.1  & \textbf{72.7} & \textbf{70.3} \\ 
                    & \bbsshort{} & 10.9 & 5.5  & 15.3 & 0.2   & 0.1  & 6.4  & 76.7 & 77.0 & 60.4 & \textbf{46.9}   & 78.8 & \textbf{84.9} & 51.0  & 68.3  & 79.6 & 78.7  & 73.1   & 44.5  & \textbf{67.6}  & \textbf{83.6}  & 72.4 & 69.6 \\ %\cline{2-24} 
                    & \bbs{}      & 21.0 & 22.0 & 19.1 & 0.5   & 0.0  & 12.5 & 73.4 & 67.5 & 56.8 & 41.2   & 77.1 & 81.6 & 45.5  & 62.1  & 74.6 & 78.9  & 67.9   & 37.8  & 54.1  & 76.4  & 71.9 & 64.4 \\ %\cline{2-24} 
                    & \Ours{}     & \textbf{26.1} & \textbf{19.1} & \textbf{40.7} & \textbf{20.4}  & \textbf{27.1} & \textbf{26.7} & 73.6 & 73.1 & 56.7 & 41.6   & 76.1 & 78.7 & 42.6  & 66.8  & 72.0 & 77.7  & 68.5   & 42.0  & 57.1  & 74.7  & 70.7 & 64.8 \\ \midrule
\multirow{4}{*}{10} & \bs{}       & 0.0  & 0.0  & 0.0  & 0.0   & 9.1  & 1.8  & 76.9 & \textbf{77.1} & \textbf{62.2} & \textbf{47.3}   & \textbf{79.4} & \textbf{85.1} & \textbf{51.3}  & \textbf{70.1}  & \textbf{78.6} & 78.0  & \textbf{75.2}   & \textbf{47.4}  & 63.9  & \textbf{85.0}  & \textbf{72.3} & \textbf{70.0} \\ %\cline{2-24} 
                    & \bbsshort{} & 11.4 & 28.4 & 8.9  & 4.8   & 7.8  & 12.2 & \textbf{77.4} & 76.9 & 60.9 & 44.8   & 78.3 & 83.2 & 48.5  & 68.9  & 78.5 & 78.9  & 72.6   & 44.8  & \textbf{67.3}  & 82.7  & 69.3 & 68.9 \\ %\cline{2-24} 
                    & \bbs{}      & 22.3 & 53.9 & 32.9 & 40.8  & 43.2 & 38.6 & 71.9 & 69.8 & 57.1 & 41.0   & 76.9 & 81.7 & 43.6  & 65.3  & 77.3 & \textbf{79.2}  & 70.1   & 41.5  & 63.7  & 76.9  & 69.1 & 65.7 \\ %\cline{2-24} 
                    & \Ours       & \textbf{30.0} & \textbf{62.7} & \textbf{43.2} & \textbf{60.6}  & \textbf{39.6} & \textbf{47.2} & 65.3 & 73.5 & 54.7 & 39.5   & 75.7 & 81.1 & 35.3  & 62.5  & 72.8 & 78.8  & 68.6   & 41.5  & 59.2  & 76.2  & 69.2 & 63.6 \\ \midrule
% Full                &             & 73.4 & 78.6 & 77.6 & 78.8  & 70.7 & 75.9 & 77.9 & 78.3 & 64.4 & 45.6   & 81.8 & 87.4 & 54.0  & 71.6  & 82.0 & 80.2  & 74.6   & 47.6  & 73.8  & 83.6  & 73.1 & 71.8 \\
% \bottomrule
\end{tabular}
\caption{Detection performance (AP) for the base and novel categories on the PASCAL VOC dataset for the first base/novel split. We evaluate the performance for different numbers of training examples for the novel categories. }
\vspace{-3mm}
\label{tab:detail}
\end{table*}

